Fault in your stars: An Analysis of Android App Reviews

Mobile app distribution platforms such as Google Play Store allow users to share their feedback about downloaded apps in the form of a review comment and a corresponding star rating. Typically, the star rating ranges from one to five stars, with one star denoting a high sense of dissatisfaction with the app and five stars denoting a high sense of satisfaction. Unfortunately, due to a variety of reasons, often the star rating provided by a user is inconsistent with the opinion expressed in the review. For example, consider the following review for the Facebook App on Android; "Awesome App". One would reasonably expect the rating for this review to be five stars, but the actual rating is one star! Such inconsistent ratings can lead to a deflated (or inflated) overall average rating of an app which can affect user downloads, as typically users look at the average star ratings while making a decision on downloading an app. Also, the app developers receive a biased feedback about the application that does not represent ground reality. This is especially significant for small apps with a few thousand downloads as even a small number of mismatched reviews can bring down the average rating drastically. In this paper, we conducted a study on this review-rating mismatch problem. We manually examined 8600 reviews from 10 popular Android apps and found that 20% of the ratings in our dataset were inconsistent with the review. Further, we developed three systems; two of which were based on traditional machine learning and one on deep learning to automatically identify reviews whose rating did not match with the opinion expressed in the review. Our deep learning system performed the best and had an accuracy of 92% in identifying the correct star rating to be associated with a given review.

==> citesort.tex <==
%NAME: citesort.sty
% A replacement for \@citex which sorts citation numbers as well as
% compressing and allowing breaks.  Based on cite.sty by Donald
% Arseneau.
%
% for use in LaTeX say, \documentstyle[...,citesort,...]{...}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     Allow, but strongly discourage, line breaks within a long
%     series of citations.  Compress lists of successive numbers
%     to one number range, e.g., 5,6,7,8,9 --> 5--9.  Compatible
%     with versions of \@cite that use exponents.
%              -- Donald Arseneau  1989
%
% Modified to sort the numbers so they come out in increasing order,
% regardless of the way they appear in the source. O(N^2) sort!
% Ian Green, CUED, 10-Dec-1991.  Improvements to img@eng.cam.ac.uk
% please. Version 1

\newcount\@minsofar
\newcount\@min
\newcount\@cite@temp
\def\@citex[#1]#2{%
\if@filesw \immediate \write \@auxout {\string \citation {#2}}\fi
\@tempcntb\m@ne \let\@h@ld\relax \def\@citea{}%
\@min\m@ne%
\@cite{%
  \@for \@citeb:=#2\do {\@ifundefined {b@\@citeb}%
    {\@h@ld\@citea\@tempcntb\m@ne{\bf ?}%
    \@warning {Citation `\@citeb ' on page \thepage \space undefined}}%
{\@minsofar\z@ \@for \@scan@cites:=#2\do {%
  \@ifundefined{b@\@scan@cites}%
    {\@cite@temp\m@ne}
    {\@cite@temp\number\csname b@\@scan@cites \endcsname \relax}%
\ifnum\@cite@temp > \@min% select the next one to list
    \ifnum\@minsofar = \z@
      \@minsofar\number\@cite@temp
      \edef\@scan@copy{\@scan@cites}\else
    \ifnum\@cite@temp < \@minsofar
      \@minsofar\number\@cite@temp
      \edef\@scan@copy{\@scan@cites}\fi\fi\fi}\@tempcnta\@min
  \ifnum\@minsofar > \z@ % some more
    \advance\@tempcnta\@ne
    \@min\@minsofar
    \ifnum\@tempcnta=\@minsofar %   Number follows previous--hold on to it
      \ifx\@h@ld\relax
        \edef \@h@ld{\@citea\csname b@\@scan@copy\endcsname}%
      \else \edef\@h@ld{\ifmmode{-}\else--\fi\csname b@\@scan@copy\endcsname}%
      \fi
    \else \@h@ld\@citea\csname b@\@scan@copy\endcsname
          \let\@h@ld\relax
  \fi % no more
\fi}%
\def\@citea{,\penalty\@highpenalty\,}}\@h@ld}{#1}}

% end of citesort.sty

==> future.tex <==
% future.tex

Intuition and experience strongly suggest that users look at the average rating of an
app before making a decision on downloading it. Studies also confirm that average rating
of an app heavily influences the number of downloads of the app. However, 
we believe that the notion of average rating needs to be refined. As it stands now, it
can easily be inflated or deflated and may not represent the actual feedback of the users.

The first step towards refining this average rating is to detect inconsistencies between
the opinion expressed in the review and the rating given. We have proposed automated approaches to solve this problem in the current paper. 

However, other refinements are possible to this notion of average rating
and can be the subject of extensive future work. In statistics, we have the notion of Cohen's Kappa to measure inter-annotator agreement. It not only factors in the agreement among the annotators but also factors in agreement by chance, by using the probability of an annotator giving a particular annotation. Similarly, we will need to factor in whether a user is generally disposed to rating apps high, say, five stars (or conversely, generally disposed to rating low, say, one star).

\begin{comment}
Further, in our interview with end users who participated in our evaluation, some users said that although they had several complaints about a particular app, they still rated it high as there were no competing apps. A more sophisticated average rating system should also factor in the uniqueness of the app, for which, we may need some kind of a uniqueness or singularity metric.
\end{comment}
